Mosaic-SDF for 3D Generative Models

Current diffusion or flow-based generative models for 3D shapes divide to two: distilling pre-trained 2D image diffusion models, and training directly on 3D shapes. When training a diffusion or flow models on 3D shapes a crucial design choice is the shape representation. An effective shape representation needs to adhere three design principles: it should allow an efficient conversion of large 3D datasets to the representation form; it should provide a good tradeoff of approximation power versus number of parameters; and it should have a simple tensorial form that is compatible with existing powerful neural architectures. While standard 3D shape representations such as volumetric grids and point clouds do not adhere to all these principles simultaneously, we advocate in this paper a new representation that does. We introduce Mosaic-SDF (M-SDF): a simple 3D shape representation that approximates the Signed Distance Function (SDF) of a given shape by using a set of local grids spread near the shape's boundary. The M-SDF representation is fast to compute for each shape individually making it readily parallelizable; it is parameter efficient as it only covers the space around the shape's boundary; and it has a simple matrix form, compatible with Transformer-based architectures. We demonstrate the efficacy of the M-SDF representation by using it to train a 3D generative flow model including class-conditioned generation with the 3D Warehouse dataset, and text-to-3D generation using a dataset of about 600k caption-shape pairs.

==> tables/representations_comparison.tex <==
% \begin{table*}[h]
% % \renewcommand{\tabcolsep}{1.0pt}
% \begin{tabular}{@{}l|cccc}
% \textbf{Representation} & Grid-based & Point Cloud  & Implicit Neural & \emph{Point-Based Implicit} \\ \hline
% Expressiveness & \cmark & \xmark & \cmark & \cmark \\ 
% Parameter efficient & \xmark & \xmark & \cmark & \cmark \\ 
% Pre-process time & \xmark & \cmark & \xmark & \cmark \\ 
% Compatible architecture & \cmark & \cmark & \xmark & \cmark \\ 
% Spatial invariance &  \cmark & \cmark & \xmark & \cmark \\ \hline
%  \end{tabular}
% \caption{
% Comparison of existing 3D representation used for generation.
% \ly{edit the categories, maybe add citations to each representation}}
% \label{tab:rep_comp}
% \end{table*}

\begin{table*}[h]
% \renewcommand{\tabcolsep}{1.0pt}
\begin{tabular}{@{}lccc}
\toprule
\textbf{Representation} & Volumetric grid & Implicit Neural & M-SDF \\ \midrule
Pre-process (1 shape) & 30sec & 1 hr & 2min \\  
SDF approximation & XXX & XXX & XXX  \\ 
Inference (1 point)  & XXX & XXX & XXX \\ 
Tensorial structure & trans & perm$\times\cdots\times$perm  & perm$\times$trans \\ \bottomrule
 \end{tabular}
\caption{
Comparison of 3D representation that allow single shape \yl{XXX}.
\ly{edit the categories, maybe add citations to each representation}}
\label{tab:rep_comp}
\end{table*}

==> tables/shapenet_eval.tex <==
\renewcommand{\arraystretch}{1.1} % Adjust the value as needed
% \renewcommand{\tabcolsep}{1.0pt}
\begin{table}[h]
    \centering
    \resizebox{1.\linewidth}{!}{
    \begin{tabular}{lcccccccc} 
     \toprule
       &  FPD ($\downarrow$) & KPD ($\downarrow$) &  \multicolumn{2}{c}{MMD ($\downarrow$)} & \multicolumn{2}{c}{COV ($\uparrow$,\%)} & \multicolumn{2}{c}{1-NNA ($\downarrow$,\%)}\\
       &   &  &  \small{CD}  & \small{EMD} & \small{CD} & \small{EMD} & \small{CD} & \small{EMD} \\
       \bottomrule
       airplane & & & & & & & &
      % MMD-CD ($\downarrow$) & MMD-EMD ($\downarrow$) & COV-CD ($\uparrow$) & COV-EMD ($\uparrow$)
      \\ \midrule % \Xhline{1pt}
     \textbf{\textit{3DILG}} \ 
    &
    $1.83$
     &
    $3.22$
    &
    $4.69$
    &
    $4.73$
    &
    $41.09$
    &
    $32.67$
    &
    $82.67$
    &
    $84.41$
    \\
      \textbf{\textit{Neural Wavelet}} \ 
     &
    $0.81$
    &
    $1.26$
    &
    $3.36$
    &
    $4.19$
    &
    $51.98$
    &
    $45.05$
    &
    $68.32$
    &
    $73.76$
    \\
     \textbf{\textit{3DShape2VecSet}} \ 
     &
    $0.94$
    &
    $1.65$
    &
    $3.80$
    &
    $4.45$
    &
    $51.98$
    &
    $40.59$
    &
    $69.06$
    &
    $76.73$
    \\
     \rowcolor{lightgray}
      \textbf{\textit{Ours}} \ 
     &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    \\
     \bottomrule %\Xhline{1pt} 
      car &   &  &  &  &   &  &  & 
      \\ \midrule % \Xhline{1pt}
     \textbf{\textit{3DILG}} \ 
     &
    $2.84$
    &
    $6.24$
    &
    $4.67$
    &
    $3.83$
    &
    $18.86$
    &
    $20.57$
    &
    $93.43$
    &
    $90.57$
    \\
     \textbf{\textit{Neural Wavelet}} \ 
     &
    -
    &
    -
    &
    -
    &
    -
    &
    -
    &
    -
    &
    -
    &
    -
    \\
     \textbf{\textit{3DShape2VecSet}} \ 
     &
    $1.32$
    &
    $2.17$
    &
    $4.13$
    &
    $3.52$
    &
    $37.71$
    &
    $40.00$
    &
    $84.57$
    &
    $86.57$
    \\
    \rowcolor{lightgray}
     \textbf{\textit{Ours}} \ 
     &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    \\
     \bottomrule %\Xhline{1pt} 
           chair &   &  &  &  &   &  &  & 
      \\ \midrule % \Xhline{1pt}
     \textbf{\textit{3DILG}} \ 
     &
    $1.64$
    &
    $1.20$
    &
    $20.37$
    &
    $10.54$
    &
    $37.87$
    &
    $39.94$
    &
    $74.11$
    &
    $69.38$
    \\
     \textbf{\textit{Neural Wavelet}} \ 
    &
    $1.41$
    &
    $1.29$
    &
    $16.53$
    &
    $9.47$
    &
    $43.79$
    &
    $47.04$
    &
    $59.47$
    &
    $64.20$
    \\
     \textbf{\textit{3DShape2VecSet}} \ 
     &
    $0.77$
    &
    $0.63$
    &
    $16.97$
    &
    $9.44$
    &
    $51.78$
    &
    $52.37$
    &
    $58.43$
    &
    $60.80$
    \\
    \rowcolor{lightgray}
     \textbf{\textit{Ours}} \ 
     &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    \\
     \bottomrule %\Xhline{1pt} 
                sofa &   &  &  &  &   &  &  & 
      \\ \midrule % \Xhline{1pt}
     \textbf{\textit{3DILG}} \ 
     &
    $3.19$
    &
    $5.83$
    &
    $26.41$
    &
    $10.71$
    &
    $25.95$
    &
    $29.11$
    &
    $84.81$
    &
    $77.85$
    \\
     \textbf{\textit{Neural Wavelet}} \ 
     &
    -
    &
    -
    &
    -
    &
    -
    &
    -
    &
    -
    &
    -
    &
    -
    \\
     \textbf{\textit{3DShape2VecSet}} \ 
     &
    $1.17$
    &
    $1.70$
    &
    $10.83$
    &
    $7.25$
    &
    $48.73$
    &
    $51.90$
    &
    $62.66$
    &
    $57.91$
    \\
    \rowcolor{lightgray}
     \textbf{\textit{Ours}} \ 
     &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    \\
     \bottomrule %\Xhline{1pt}
           table &   &  &  &  &   &  &  & 
      \\ \midrule % \Xhline{1pt}
     \textbf{\textit{3DILG}} \ 
     &
    $2.86$
    &
    $4.13$
    &
    $22.96$
    &
    $10.18$
    &
    $29.45$
    &
    $30.88$
    &
    $78.27$
    &
    $78.74$
    \\
     \textbf{\textit{Neural Wavelet}} \ 
     &
    $1.49$
    &
    $2.20$
    &
    $13.27$
    &
    $7.72$
    &
    $51.07$
    &
    $47.98$
    &
    $56.41$
    &
    $58.67$
    \\
     \textbf{\textit{3DShape2VecSet}} \ 
     &
    $0.83$
    &
    $0.92$
    &
    $14.06$
    &
    $8.01$
    &
    $53.44$
    &
    $49.41$
    &
    $59.74$
    &
    $61.05$
    \\
    \rowcolor{lightgray}
     \textbf{\textit{Ours}} \ 
     &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    &
    $X$
    \\
     \bottomrule %\Xhline{1pt}  
    \end{tabular} } 
    \caption{Evaluation of our class conditioning generation model trained on ShapenetCore v2 \cite{shapenet2015} \ly{XXX name?} compared to baselines. We report results on the 5 largest classes in the dataset. KPD is multiplied by $10^3$, MMD-CD is multiplied by $10^3$ and MMD-EMD is multiplied by $10^2$.
    \ly{XXX fill in the numbers}
    }\label{tab:shapenet_cond}
\end{table}
